SequentialAttention++ for Block Sparsification: Differentiable Pruning Meets Combinatorial Optimization

Neural network pruning is a key technique towards engineering large yet scalable, interpretable, and generalizable models. Prior work on the subject has developed largely along two orthogonal directions: (1) differentiable pruning for efficiently and accurately scoring the importance of parameters, and (2) combinatorial optimization for efficiently searching over the space of sparse models. We unite the two approaches, both theoretically and empirically, to produce a coherent framework for structured neural network pruning in which differentiable pruning guides combinatorial optimization algorithms to select the most important sparse set of parameters. Theoretically, we show how many existing differentiable pruning techniques can be understood as nonconvex regularization for group sparse optimization, and prove that for a wide class of nonconvex regularizers, the global optimum is unique, group-sparse, and provably yields an approximate solution to a sparse convex optimization problem. The resulting algorithm that we propose, SequentialAttention++, advances the state of the art in large-scale neural network block-wise pruning tasks on the ImageNet and Criteo datasets.

==> algorithm.tex <==
\section{The SequentialAttention++ algorithm}
\label{sec:algorithm}

As discussed, the basic form of 
SequentialAttention++ is a 
combination of Sequential Attention and ACDC. More specifically,
we first introduce the sequential attention parameterization, 
where we multiply each selection candidate (e.g. block, in the case of block sparsification) by a trainable attention weight.
Then, we employ the alternating compressed and decompressed
phases of ACDC \emph{on the attention weights} (instead of doing so on the selection candidates' weights themselves). This 
helps factor out the inherent magnitude differences between
model parameters, which do not necessarily correlate with
importances. The basic algorithm can be seen in Algorithm~\ref{alg:example}.

\begin{algorithm}[tb]
   \caption{Feed-forward layer with the basic version of SequentialAttention++ to select top $k$ parameters from a kernel $\bfW$. We omit $\textsc{sparsification}$ phases for simplicity.}
   \label{alg:example}
\begin{algorithmic}
\FUNCTION{$\text{FF}({{\bf X}\in \mathbb{R}^{b\times n}}: \text{input batch}, t:\text{training step})$}
   \STATE Trainable params:
   \STATE Kernel matrix ${\bf W}\in\mathbb{R}^{n\times m}$, Logits ${\bf L}\in\mathbb{R}^{n\times m}$
   \STATE 
   \STATE ${\bf A} = nm \cdot e^{\bf L}/\sum e^{\bf L}$
   \STATE ${\bf \hat{W}} = {\bf W} \odot {\bf A} \odot \text{Mask}({\bf A}, t)$
   \STATE {\bf return} ${\bf X} {\bf \hat{W}}$
\ENDFUNCTION
\STATE 
\FUNCTION{$\text{Mask}({\bf A}:\text{attention weights}, t:\text{training step})$}
    \STATE Non-trainable state: $\text{mask}\in\{0,1\}^{n\times m}$
    \STATE 
    \IF{$t$ is in a $\textsc{dense}$ phase}
        \STATE $\text{mask} \leftarrow \text{top}_k({\bf A})$
        \STATE {\bf return} ${\bf 1}_{n\times m}$
    \ELSIF{$t$ is in a $\textsc{sparse}$ phase}
        \STATE {\bf return} $\text{mask}$
    \ENDIF
\ENDFUNCTION
\end{algorithmic}

\end{algorithm}

\subsection{The $\textsc{sparsification}$ phase}
\label{sec:sparsification}

One drawback of sparse/dense phases is that the dense-to-sparse
transition is abrupt. Since the lowest-magnitude weights
are instantly pruned, this neglects correlations between
these pruned parameters. If we were to re-train
the model after pruning one parameter at a time, the picture
could be drastically different, since low-magnitude weights
could grow (this could happen e.g. due to parameter 
redundancy). In fact, this effect was highlighted by \citet{kuznedelev2023cap}, who devised a backward selection 
method based on correlations as captured by the Hessian.

Inspired by this approach, we incorporate a backward selection
phase between the $\textsc{dense}$ and $\textsc{sparse}$ phases,
which we call the $\textsc{sparsification}$ phase. In this 
phase, we gradually prune the least important features based on
the attention weights. This gradual process allows the model
to re-adjust the attention weights after some parameters are
pruned. The importance of this phase is validated using ablation experiments in
Appendix~\ref{sec:ablation_sparsification}.
We use an exponential pruning schedule, to prune more
aggressively in the beginning of the phase, and more carefully
at the end (as we approach the desired number of candidates 
$k$). A comparison of the sparsity schedules of ACDC and SequentialAttention++ can be found in Figure \ref{fig:sparse_step}. We use the sparsity schedule
$\text{sparsity}(t) = s \cdot \frac{1-e^{-ct}}{1-e^{-c}}$ for $t\in[0,1]$, where $s$ is the target sparsity. This interpolates
between sparsity $0$ and $s$, and constitutes a single
$\textsc{sparsification}$ phase. We choose the constant $c=4$ (for an ablation 
analysis, see Appendix~\ref{sec:ablation_rampup_factor}).

\begin{figure}[tb]
    \label{fig:sparse_step}
    \centering
    % \includegraphics[width=0.7\linewidth]{figures/sparse_step.pdf}
    \includegraphics[width=0.5\linewidth]{figures/sparse_step.pdf}
    \caption{Sparsity schedules of ACDC and SequentialAttention++. ACDC uses an instant dense-to-sparse
    transition, while SequentialAttention++ uses an
    exponential sparsity schedule.}
\end{figure}

